Entropy Coding Improvement for Low-complexity Compressive Auto-encoders

End-to-end image and video compression using auto-encoders (AE) offers new appealing perspectives in terms of rate-distortion gains and applications. While most complex models are on par with the latest compression standard like VVC/H.266 on objective metrics, practical implementation and complexity remain strong issues for real-world applications. In this paper, we propose a practical implementation suitable for realistic applications, leading to a low-complexity model. We demonstrate that some gains can be achieved on top of a state-of-the-art low-complexity AE, even when using simpler implementation. Improvements include off-training entropy coding improvement and encoder side Rate Distortion Optimized Quantization. Results show a 19% improvement in BDrate on basic implementation of fully-factorized model, and 15.3% improvement compared to the original implementation. The proposed implementation also allows a direct integration of such approaches on a variety of platforms.

==> Makefile <==
FILENAME = dcc_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done


==> implem.tex <==
\section{Practical Implementation}

%gdn->relu, float->int, auto-regressive-> context switch, python -> SADL C++ imple

%Video compression systems, in particular decoders embedded in low-end devices such as smartphone or set-top-boxes for instance, need to be capable to process videos of increasing resolutions and framerates, involving extremely challenging computational complexity and memory management. Despite the rise and rapid improvement of graphical process units, which enable the use of highly parallelized floating-point operations in deep neural networks, lightweight decoder architectures is key for potential deployment in the foreseeable future






==> training.tex <==
\subsection{Training}

We consider a pre-selected number of epochs for training: $number\_of\_epochs$. At a given epoch, \textit{e.g.,} $number\_of\_epoch/2$, the weights and biases of the decoder layers are quantized and frozen as described below. The weights and biases of the deconvolutional layers of the decoder will not change anymore until the end of the training.
However, the weights and biases of the encoder layers will continue to be updated until the end the training at $number\_of\_epoch$. By freezing the update of the weights and biases of deconvolutional layers and by continuing the update of weights and biases of the convolutional layers of the encoder, the encoder will compensate the distortion induced by the quantization and the Loss will continue to decrease until the end of the training.
We can freeze using different strategies:
\begin{itemize}
 \item	We freeze all decoding layers at the same time, at the same epoch, \textit{e.g.} $number\_of\_epoch/2$
 \item	We freeze each $deconv_i$ of the decoder at different epochs. The most important layer in terms of impact on the reconstruction performance is the last layer $deconv_3$, i.e., the closest to the output. Hence, we start by freezing this layer $deconv_3$ and continue until layer $deconv_0$, the closest to the entropy decoder. For instance, we present the following scheduling:
\begin{itemize}
	\item At $number\_of\_epoch/2$, $deconv_3$ is frozen
	\item At $5*number\_of\_epoch/8$, $deconv_2$ is frozen
	\item At $6*number\_of\_epoch/8$, $deconv_1$ is frozen
	\item At $7*number\_of\_epoch/8$, $deconv_0$ is frozen
\end{itemize}
\end{itemize}

% , authors explained that ANNs, based on floating point math, can lead to strong failure when deployed on heterogeneous platform such as embedded platform. They propose to use integer arithmetic in these ANNs. They present a quantized network, so called integer network. The gradient is computed and kept in floating point while the weights are quantized. 
% The main drawback is the usage of integer network for both coder and decoder while in some cases the integer decoder is enough and needs to be tuned for heterogenous platform.
%\hfill \break
\textcolor{red}{Franck: not sure we need this: this is very torch specific stuff. Better explain the overall quantizer proxy we use (quantif 2N- clip - dequantif)}

%To target heterogeneous platform and to obtain a quantized network, we propose to quantize and freeze the convolutional layers $g_s$ during the training stage. The parameters of the decoder neural networks are quantized with n-bits of precision, e.g int16, but still temporarily stored as float for floating point operations during the training stage. The quantization range is:
%\begin{align*}
%\left[(-2)^{nbits-1},(+2)^{nbits+1}\right] \\
%quantizer=2^n
%\end{align*}
%Then, the matrix $X=\{deconv_i \}_{(i=0..3)}$  is quantized as follows :
%\begin{align*}
%X_{quant}&=newround(X*quantizer)\\
%X_{new}&=X_{quant}/quantizer
%\end{align*}
%where
%\begin{align*}
%newround()= (torch.round(x) - x).detach() + x
%\end{align*}
%defined using Torch backend. Indeed, a uniform quantization is thus defined that it is differentiable in case of forward or backward propagation. The classical round() function, used in uniform quantization, is gradient NULL. Function that returns gradient NULL cannot be used in backward propagation. Said otherwise, a network will not learn anything in the case where a NULL gradient is returned. A workaround is to use the straight-through estimator (STE) \cite{Bengio13ste} so that the gradient becomes non-NULL. STE ignores the derivative of the round() function and passes on the incoming gradient as if the function was an identity function.
%\newline
%Let $nbits$ set to $16$ the n-bits of precision to quantize into $int16$. $X_{quant}$ is the quantized version of $X$ and $X_{new}$ is used temporarily to go back as float for floating point operations during the training stage.
%\newline
%In a first approach, the same quantizer is thus used for all deconvolutional layers $deconv_i$: 
%\begin{align*}
%deconv_i=  newround(deconv_i*quantizer)/quantizer
%\end{align*}
%with             
%\begin{align*}
%quantizer= 2^n \\
%n=nbits-1-\lceil log_2(max(\rvert X\rvert)) \rceil
%\end{align*}

%For $int16$ quantization we have:
%\begin{align*}
%(deconv_i)_{ int16}=newround(deconv_i*2^n)\\
%n=15-\lceil log_2(max(\rvert \{deconv_i\}\rvert)) \rceil
%\end{align*}

%In this case the quantizer is stored and transmitted to the decoder. The weights and biases of each $deconv_i$ are quantized using the same quantizer $(deconv_i*quantizer)$ and transmitted to the decoder for inference. During the inference, all the operations are performed in integer and the outputs of each $deconv_i$ are clamped to $\left[(-2)^{nbits-1},(+2)^{nbits+1}\right]$. At the end of decoding, the output is finally rescaled to the initial range (e.g.  $\left[0,256 \right]$ if output images are in 8 bits) using quantizer. 

%In a variant approach, a quantizer is set for each deconvolutional layer $deconv_i$. 
%\begin{align*}
%deconv_i=  newround(deconv_i*quantizer_i )/quantizer_i 
%\end{align*}
%With             
%\begin{align*}
%quantizer_i= 2^{n_i} \\
%n_i=nbits-1-\lceil log_2(max(\rvert deconv_i\rvert))\rceil
%\end{align*}
%In this case the $\{quantizer_i\}$ are stored and transmitted to the decoder.

% NO The decoder applies a dequantizer to each deconvolutional layer $deconv_i$ using the associated transmitted quantizer $quantizer_i$  during the inference decoding stage. 

